Unsupervised Domain Generalization by Learning a Bridge Across Domains

The ability to generalize learned representations across significantly different visual domains, such as between real photos, clipart, paintings, and sketches, is a fundamental capacity of the human visual system. In this paper, different from most cross-domain works that utilize some (or full) source domain supervision, we approach a relatively new and very practical Unsupervised Domain Generalization (UDG) setup of having no training supervision in neither source nor target domains. Our approach is based on self-supervised learning of a Bridge Across Domains (BrAD) - an auxiliary bridge domain accompanied by a set of semantics preserving visual (image-to-image) mappings to BrAD from each of the training domains. The BrAD and mappings to it are learned jointly (end-to-end) with a contrastive self-supervised representation model that semantically aligns each of the domains to its BrAD-projection, and hence implicitly drives all the domains (seen or unseen) to semantically align to each other. In this work, we show how using an edge-regularized BrAD our approach achieves significant gains across multiple benchmarks and a range of tasks, including UDG, Few-shot UDA, and unsupervised generalization across multi-domain datasets (including generalization to unseen domains and classes).

==> demo_figures/demo_aircraft_carrier.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_aircraft_carrier.png}
    \caption{\democap{Aircraft Carrier}}
    \label{fig:demo_aircraft_carrier}
\end{figure*}


==> demo_figures/demo_cat.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_cat.png}
    \caption{\democap{Cat}}
    \label{fig:demo_cat}
\end{figure*}

==> demo_figures/demo_coffee_cup.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_coffee_cup.png}
    \caption{\democap{Coffee Cup}}
    \label{fig:demo_coffee_cup}
\end{figure*}


==> demo_figures/demo_crocodile.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_crocodile.png}
    \caption{\democap{Crocodile}}
    \label{fig:demo_crocodile}
\end{figure*} 

==> demo_figures/demo_duck.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_duck.png}
    \caption{\democap{Duck}}
    \label{fig:demo_duck}
\end{figure*} 


==> demo_figures/demo_eyeglasses.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_eyeglasses.png}
    \caption{\democap{Eyeglasses}}
    \label{fig:demo_eyeglasses}
\end{figure*}


==> demo_figures/demo_fork.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{demo_figures/demo_fork.png}
    \caption{\democap{Fork}}
    \label{fig:demo_fork}
\end{figure*}


==> demo_figures/demo_gotee.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{demo_figures/demo_gotee.png}
    \caption{\democap{Gotee}}
    \label{fig:demo_gotee}
\end{figure*}


==> demo_figures/demo_helmet.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{demo_figures/demo_helmet.png}
    \caption{\democap{Helmet}}
    \label{fig:demo_helmet}
\end{figure*} 

==> demo_figures/demo_hot_dog.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth,]{demo_figures/demo_hot_dog.png}
    \caption{\democap{Hot Dog}}
    \label{fig:demo_hot_dog}
\end{figure*}


==> demo_figures/demo_lobster.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_lobster.png}
    \caption{\democap{Lobster}}
    \label{fig:demo_lobster}
\end{figure*} 

==> demo_figures/demo_monkey.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_monkey.png}
    \caption{\democap{Monkey}}
    \label{fig:demo_monkey}
\end{figure*}


==> demo_figures/demo_panda.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_panda.png}
    \caption{\democap{Panda}}
    \label{fig:demo_panda}
\end{figure*}


==> demo_figures/demo_peanut.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_peanut.png}
    \caption{\democap{Peanut}}
    \label{fig:demo_peanut}
\end{figure*} 

==> demo_figures/demo_school_bus.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_school_bus.png}
    \caption{\democap{School Bus}}
    \label{fig:demo_school_bus}
\end{figure*} 

==> demo_figures/demo_watermelon.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{demo_figures/demo_watermelon.png}
    \caption{\democap{Watermelon}}
    \label{fig:demo_watermelon}
\end{figure*}


==> figures/edge_images/edge_map_1col.tex <==
\newcommand*\figsizecol{0.3\columnwidth}
\newcommand*\trimall{0.5}

\begin{figure}[t]
\vspace{-0.4cm}
    \centering
    ~~~~~Real~~~~~~~~~~~~~~~~~~Art~~~~~~~~~~~~~~~~~~~~Sketch\\
    \rotatebox{90}{~~~~~Original}~\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_orig.png}
    \includegraphics[width=\figsizecol]{figures/edge_images/bus_art_orig.png}
    \includegraphics[width=\figsizecol]{figures/edge_images/radio_sketch_orig.png}\\
    \rotatebox{90}{~~~~~~Canny \cite{canny1986computational}}~\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_canny.png}
    \includegraphics[width=\figsizecol]{figures/edge_images/bus_art_canny.jpg}
    \includegraphics[width=\figsizecol]{figures/edge_images/radio_sketch_canny.jpg}\\
    \rotatebox{90}{~~~~~HED~Zoom~~~~~~~~~~~~~HED\cite{Xie_2015_ICCV}}~\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_hed_zoom.png}
    \includegraphics[width=\figsizecol]{figures/edge_images/bus_art_hed_zoom.png}
    \includegraphics[width=\figsizecol]{figures/edge_images/radio_sketch_hed_zoom.png}\\
    \hspace{4.5pt}\rotatebox{90}{~~~\ours{}~Zoom~~~~~~~~~~~~~~~~~\ours}~\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_per_zoom.png}
    \includegraphics[width=\figsizecol]{figures/edge_images/bus_art_per_zoom.png}
    \includegraphics[width=\figsizecol]{figures/edge_images/radio_sketch_per_zoom.png}
    \vspace{-0.2cm}
    \caption{Edge images for different choices of $\Psi_n$: (i) Canny produces noisy images with many irrelevant edges; (ii) the HED mostly outlines the object and discards important internal texture; (iii) learned $\Psi_n$ keep the informative edges and the fine internal details while discarding most of the noise.}
    \label{fig:edges_1col}
    \figvspace
\end{figure}

% Before adding zoom:


%\begin{figure}[t]
%    \centering
    % ~~~~~Real~~~~~~~~~~~~~~~~~~Art~~~~~~~~~~~~~~~~~~~~Sketch\\
    % \rotatebox{90}{~~~~~Original}~\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_orig.png}
    % \includegraphics[width=\figsizecol]{figures/edge_images/bus_art_orig.png}
    % \includegraphics[width=\figsizecol]{figures/edge_images/radio_sketch_orig.png}\\
    % \rotatebox{90}{~~~~~~Canny \cite{canny1986computational}}~\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_canny.png}
    % \includegraphics[width=\figsizecol]{figures/edge_images/bus_art_canny.jpg}
    % \includegraphics[width=\figsizecol]{figures/edge_images/radio_sketch_canny.jpg}\\
    % \rotatebox{90}{~~~~~~~HED\cite{Xie_2015_ICCV}}~\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_hed.png}
    % \includegraphics[width=\figsizecol]{figures/edge_images/bus_art_hed.png}
    % \includegraphics[width=\figsizecol]{figures/edge_images/radio_sketch_hed.png}\\
    % \rotatebox{90}{~~~~~~~~~\ours}~\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_per.png}
    % \includegraphics[width=\figsizecol]{figures/edge_images/bus_art_per.png}
    % \includegraphics[width=\figsizecol]{figures/edge_images/radio_sketch_per.png}
    % \caption{Edge images for different choices of $\Psi_k$: (i) Canny produces noisy images with many irrelevant edges; (ii) the HED mostly outlines the object and discards important internal texture; (iii) learned $\Psi_k$ keep the informative edges and the fine internal details while discarding most of the noise.}
    % \label{fig:edges_1col}
    % \figvspace
% \end{figure}


%\begin{figure}
%    \centering
%    ~~~~~~~Real~~~~~~~~~~~~~~~~~~Real~~~~~~~~~~~~~~~~Art~~~~~~~~~~~~~~~~~ Clipart\\
%    \rotatebox{90}{~~~~~Original}~\includegraphics[width=\figsizecol]{figures/edge_images/horse_real_orig.png}\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_orig.png}
%    \includegraphics[width=\figsizecol]{figures/edge_images/zebra_art_orig.png}
%    \includegraphics[width=\figsizecol]{figures/edge_images/zebra_ca_orig.png}\\
%    \rotatebox{90}{~~~~~~Canny \cite{canny1986computational}}~\includegraphics[width=\figsizecol]{figures/edge_images/horse_real_canny.png}\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_canny.png}
%    \includegraphics[width=\figsizecol]{figures/edge_images/zebra_art_canny.png}
%    \includegraphics[width=\figsizecol]{figures/edge_images/zebra_ca_canny.png}\\
%    \rotatebox{90}{~~~~~~~HED\cite{Xie_2015_ICCV}}~\includegraphics[width=\figsizecol]{figures/edge_images/horse_real_hed.png}\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_hed.png}
%    \includegraphics[width=\figsizecol]{figures/edge_images/zebra_art_hed.png}
%    \includegraphics[width=\figsizecol]{figures/edge_images/zebra_ca_hed.png}\\
%    \rotatebox{90}{~~~~~~~~~\ours}~\includegraphics[width=\figsizecol]{figures/edge_images/horse_real_per.png}\includegraphics[width=\figsizecol]{figures/edge_images/zebra_real_per.png}
%    \includegraphics[width=\figsizecol]{figures/edge_images/zebra_art_per.png}
%    \includegraphics[width=\figsizecol]{figures/edge_images/zebra_ca_per.png}
%    \caption{Edge images for different selections for $\Psi_k$: We observe that the Canny output produces noisy images with many irrelevant edges. On the other hand, the HED output mostly outlines the object and discards important texture. Our proposed \ours{} keeps the informative edges and the fine details while discarding most of the noise.}
%    \label{fig:edges_1col}
%\end{figure}

==> figures/edge_images/edge_maps.tex <==
\newcommand*\figsize{0.15\textwidth}

%DomainNet

\begin{figure*}[ht]
    \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \caption{}
         \includegraphics[width=\textwidth]{figures/edge_images/car_real_orig.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \caption{}
         \includegraphics[width=\textwidth]{figures/edge_images/car_real_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \caption{}
         \includegraphics[width=\textwidth]{figures/edge_images/car_real_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \caption{}
         \includegraphics[width=\textwidth]{figures/edge_images/car_real_per.png}
    \end{subfigure}
    
    \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/bus_real_orig.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/bus_real_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/bus_real_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/bus_real_per.png}
    \end{subfigure}

             \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/bus_ca_orig.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/bus_ca_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/bus_ca_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/bus_ca_per.png}
    \end{subfigure}
    
        \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/jacket.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/jacket_ca_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/jacket_cs_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/jacket_ca_per_domain.png}
    \end{subfigure}

        \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/car_sketch_orig.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/car_sketch_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/car_sketch_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/car_sketch_per.png}
    \end{subfigure}

    \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/zebra_sketch_orig.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/zebra_sketch_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/zebra_sketch_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/zebra_sketch_per.png}
    \end{subfigure}
    

         \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/zebra_art_orig.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/zebra_art_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/zebra_art_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/zebra_art_per.png}
    \end{subfigure}



        \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/car_art_orig.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/car_art_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/car_art_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/car_art_per.png}
    \end{subfigure}


    
    \caption{Edge images in different settings. (a) Original images (b) Canny edge detector  \cite{canny1986computational} (c) Hed edge detector \cite{Xie_2015_ICCV} (d) Trainable Hed edge detector (e) BrAD trainable edge detector}
    \label{fig:edge_maps}
\end{figure*}


\begin{figure*}[ht]

     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \caption{}
         \includegraphics[width=\textwidth]{figures/edge_images/passport_real_orig.png}
     \end{subfigure}
      \centering
     \begin{subfigure}[b]{\figsize}
     \caption{}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/passport_real_canny.jpg}
     \end{subfigure}
      \centering
     \begin{subfigure}[b]{\figsize}
     \caption{}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/passport_real_hed.png}
     \end{subfigure}
      \centering
     \begin{subfigure}[b]{\figsize}
     \caption{}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/passport_real_per.png}
     \end{subfigure}

    \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/passport_sketch_orig.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/passport_sketch_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/passport_sketch_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/passport_sketch_per.png}
    \end{subfigure}
    
    \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/passport_ca_orig.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/passport_ca_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/passport_ca_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/passport_ca_per_domain.png}
    \end{subfigure}

        \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/jacket_art_orig.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/jacket_art_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/jacket_art_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/jacket_art_per.png}
    \end{subfigure}

         
         \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/radio_real_orig.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/radio_real_canny.jpg}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/radio_real_hed.png}
    \end{subfigure}
     \centering
     \begin{subfigure}[b]{\figsize}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_images/radio_real_per.png}
    \end{subfigure}

    \caption{Edge images in different settings. (a) Original images (b) Canny edge detector  \cite{canny1986computational} (c) Hed edge detector \cite{Xie_2015_ICCV} (d) Trainable Hed edge detector (e) BrAD trainable edge detector}
    \label{fig:edge_maps}
\end{figure*}


\iffalse

\fi

==> figures/localization.tex <==
\begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
        \caption{Query image}
         \includegraphics[width=\textwidth]{figures/statuscope_clipart.png}
         \label{subfig:Im11}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \caption{Search Space image}
         \includegraphics[width=\textwidth]{figures/statuscope_real.png}
         \label{subfig:Im21}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \caption{Query localization}
         \includegraphics[width=\textwidth]{figures/statuscope_loc.png}
         \label{subfig:loc1}
     \end{subfigure}
     
     \centering
     \vspace{-12}
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/spider_clipart1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/spider_real1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/spider_loc.png}
     \end{subfigure}    
    
         \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/snow_clipart.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/snow_real.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/snow_loc.png}
     \end{subfigure}    

    
             \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/wheel_clipart1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/wheel_real.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/wheel_loc.png}
     \end{subfigure}    
     
             \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/tiger_clipart.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/tiger_real.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/tiger_loc.png}
     \end{subfigure}  
     

                       \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/dress_orig.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/dress_real1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/dress_loc1.png}
     \end{subfigure}  

          
                            \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/dress_orig.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/dress1_real1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/dress1_loc1.png}
     \end{subfigure}  
     
       
 
\caption{Localization examples. The detected location of the object depicted on the query image $I_Q$ \ref{subfig:Im11} inside the different visual domain search space image $I_S$ \ref{subfig:Im21} is presented in \ref{subfig:loc1}. The opacity of each patch is depicting the probability of its corresponding feature (on the feature map $M_S$) to belong to the chosen cluster whose average feature maximally matches $F_Q$.}
\label{fig:localization1}
\end{figure}


\begin{figure}[ht]
     \centering
     \vspace{-15}
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
        \caption{Query image}
         \includegraphics[width=\textwidth]{figures/box1_clipart1.png}
         \label{subfig:Im12}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \caption{Search Space image}
         \includegraphics[width=\textwidth]{figures/box_real1.png}
         \label{subfig:Im22}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \caption{Query localization}
         \includegraphics[width=\textwidth]{figures/box_loc1.png}
         \label{subfig:loc2}
     \end{subfigure}
     
     \centering
     \vspace{-12}
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/box1_clipart1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/box1_real1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/box1_loc1.png}
     \end{subfigure}    
    
         \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/car_ca1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/car_real.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/car_loc1.png}
     \end{subfigure}    

    
             \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/hat_ca1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/hat_real.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/hat_loc.png}
     \end{subfigure}    
     
             \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/top_orig1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/top_real1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/top_loc1.png}
     \end{subfigure}  
     
                  \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/jacket_orig1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/jacket_real.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/jacket_loc1.png}
     \end{subfigure}  
     
                       \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mirror_clipart1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mirror_real.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mirror_loc.png}
     \end{subfigure}  

                                          \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/soup_ca.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/soup_real.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/soup_loc.png}
     \end{subfigure}
     
\caption{Localization examples. The detected location of the object depicted on the query image $I_Q$ \ref{subfig:Im12} inside the different visual domain search space image $I_S$ \ref{subfig:Im22} is presented in \ref{subfig:loc2}. The opacity of each patch is depicting the probability of its corresponding feature (on the feature map $M_S$) to belong to the chosen cluster whose average feature maximally matches $F_Q$.}
\label{fig:localization2}
\end{figure}

\begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
        \caption{Query image}
         \includegraphics[width=\textwidth]{figures/text1_orig1.png}
         \label{subfig:Im1}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \caption{Search Space image}
         \includegraphics[width=\textwidth]{figures/text1_real.png}
         \label{subfig:Im2}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \caption{Query localization}
         \includegraphics[width=\textwidth]{figures/text1_loc1.png}
         \label{subfig:loc}
     \end{subfigure}
     \vspace{-12}

                            \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/text1_orig1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/pure_text_real1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/pure_text_loc1.png}
     \end{subfigure}  
     
                                 \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/text_orig2.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/text_real1.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/text_loc1.png}
     \end{subfigure}  

                            \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plant.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plant_real.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/plant_loc.png}
     \end{subfigure}  
     

                           \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rocks_ca.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rocks_real.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rocks_loc.png}
     \end{subfigure}  
     


                              \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/radio_ca.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/radio_real.png}
     \end{subfigure}
    \centering
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/radio_loc.png}
     \end{subfigure}  
     
\caption{Localization examples. The detected location of the object depicted on the query image $I_Q$ \ref{subfig:Im1} inside the different visual domain search space image $I_S$ \ref{subfig:Im2} is presented in \ref{subfig:loc}. The opacity of each patch is depicting the probability of its corresponding feature (on the feature map $M_S$) to belong to the chosen cluster whose average feature maximally matches $F_Q$.}
\label{fig:localization3}
\end{figure}


==> tables/fs_uda_generalization.tex <==
\begin{table*}[ht]
    \centering
    \caption{Cross datasets. The models are trained on DomainNet and tested OfficeHome, PACS and VisDA datasets. As PCS and CDS have multiple models one for each domain pair in DomainNet, for each matching domain pairs of the test dataset we used corresponding DomainNet model, for any pair having a domain not in DomainNet, we used an ensemble of all $7$ models (a bit unfair to our single model). The reported results are average over five repetitions of each run.
    \textbf{bold} = best result, \textcolor{blue}{blue} = second best.}
    \small
    \begin{tabular}{l|ccc|ccc}
        \toprule
          &  \multicolumn{3}{c|}{1-shot test}  &  \multicolumn{3}{c}{3-shot test}\\
          Method & OfficeHome& PACS & VisDA& OfficeHome& PACS & VisDA\\
        PCS &24.7 & \textcolor{blue}{40.05}& \textcolor{blue}{42.23} &35.34&\textcolor{blue}{44.73}&50.52\\
        CDS &\textcolor{blue}{30.33}&	 {31.73}& {39.79}& \textbf{39.97}&{40.29}&\textcolor{blue}{50.46}\\ 
        \midrule
        Ours &\textbf{30.64}&	\textbf{71.57}&	\textbf{44.1}&\textcolor{blue}{38.66}&	\textbf{78.63}&	\textbf{51.1}\\
        \bottomrule

    \end{tabular}
    \label{tab:cross_dataset}
    \tabvspace
\end{table*}

% \begin{table*}[ht]
%     \centering
%     \caption{Cross datasets. The models are trained on DomainNet and tested OfficeHome, PACS and VisDA datasets. PCS has 24 models, one for each domain pair in DomainNet. In PCS 1-Shot Avg and PCS 3-Shots Avg we applied all PCS models on all domain pairs and averaged the performance. Some of the datasets' domains match those of DomainNet. In PCS 1-Shot Match and PCS 3-Shots Match we applied the matching model when possible, and used average elsewhere. The reported results are average over three repetitions of each run.
%     The best results of all methods are highlighted with the \textbf{bold} font, the second best are highlighted in \textcolor{blue}{blue}.}
%     \small
%     \begin{tabular}{l|ccc|ccc}
%         \toprule
%           &  \multicolumn{3}{c|}{1-shot test}  &  \multicolumn{3}{c}{3-shot test}\\
%           Method & OfficeHome& PACS & VisDA& OfficeHome& PACS & VisDA\\
%         \midrule
%         PCS Avg&25.52&	{39.08}&	37.76&32.30&	43.99&	43.99\\
%         %PCS 1-shot Avg&23.56&	{37.89}&	36.22& 29.85&	41.97&	42.64\\
%         %PCS 3-Shot Avg&25.52&	39.08&	37.76&32.30&	43.99&	43.99\\
%         CDS Avg &{27.70}&	32.69&	35.00& {36.59}&	39.20&	45.09\\
%         \midrule
%         PCS Match&25.52  &	\textcolor{blue}{40.05}& \textcolor{blue}{40.55}& 32.71&\textcolor{blue}{48.38}&{46.59}\\
%         %PCS 1-shot Match&24.70  &	\textcolor{blue}{40.05}& \textcolor{blue}{40.55}& 32.21&\textcolor{blue}{44.73}&{46.59}\\
%         %PCS 3-Shot Match&{25.52}&	 \textcolor{blue}{39.08}& {37.76}& {32.71}&\textcolor{blue}{48.38}&{43.43}\\ 
%         CDS Match&\textcolor{blue}{28.11}&	 {31.73}& {36.37}& \textcolor{blue}{37.10}&{40.29}&\textcolor{blue}{47.35}\\ 
%         \midrule
%         Ours &\textbf{30.64}&	\textbf{71.57}&	\textbf{44.23}&\textbf{38.66}&	\textbf{78.63}&	\textbf{49.29}\\
%         \bottomrule

%     \end{tabular}
%     \label{tab:cross_dataset}
% \end{table*}


%\begin{table*}[ht]
%    \centering
%    \caption{Cross datasets. The models are trained on DomainNet and tested OfficeHome, %PACS and VisDA datasets. PCS has 24 models, one for each domain pair in DomainNet. In PCS %1-Shot Avg and PCS 3-Shots Avg we applied all PCS models on all domain pairs and averaged %the performance. Some of the datasets' domains match those of DomainNet. In PCS 1-Shot %Match and PCS 3-Shots Match we applied the matching model when possible, and used average %elsewhere. The reported results are average over three repetitions of each run, the %standard deviation values of those tests are around 1.5\% in OfficeHome, 4.5\% in PACS and %3\% in VisDA.
%    The best results of all methods are highlighted with the \textbf{bold} font, the %second best are highlighted in \textcolor{blue}{blue}.}
%    \small
%    \begin{tabular}{l|ccc|ccc|ccc}
%       \toprule
%          &  \multicolumn{3}{c|}{1-shot test}  &  \multicolumn{3}{c|}{3-shot test} &  %\multicolumn{3}{c|}{All-shot test}  \\
%          Method & OfficeHome& PACS & VisDA& OfficeHome& PACS & VisDA& OfficeHome& PACS & %VisDA\\
%        \midrule
%        PCS 1-Shot Avg&23.25\%&	36.06\%&	35.98\%& 29.86\%&	41.12\%&	42.28\%&   %39.33\%&	47.86\%&	51.64\%\\
%        PCS 3-Shot Avg&25.17\%&	38.26\%&	37.53\%&32.36\%&	42.96\%&	43.68\%&   %\textcolor{blue}{42.15\%}&	\textcolor{blue}{50.28\%}&	54.27\%\\
%        \midrule
%        PCS 1-Shot Match&24.28  \%&	36.93\%& 39.17\%& %31.22\%&44.89\%&\textcolor{blue}{46.22\%}& 39.25\%&  49.58\%&	  54.06\%\\
%        PCS 3-Shot Match&\textcolor{blue}{25.80\%}&	 \textcolor{blue}{42.07\%}& %\textcolor{blue}{37.88\%}& \textcolor{blue}{32.63\%}&\textcolor{blue}{47.35\%}&{43.14\%}& % 40.79\%&	  47.64\%&	  \textcolor{blue}{55.98\%}\\        
%        \midrule
%        Ours &\textbf{30.99\%}&	\textbf{73.02\%}&	\textbf{44.23\%}&\textbf{38.61\%}&	%\textbf{78.71\%}&	\textbf{49.29\%}&\textbf{47.34\%}&	\textbf{80.37\%}&	%\textbf{57.60\%}\\
%        \bottomrule
%    \end{tabular}
%    \label{tab:cross_dataset}
%\end{table*}

%\begin{table*}[ht]
%    \centering
%    \caption{Cross datatsets. The models are trained on DomainNet and tested on different %datasets. }
%    \small
%    \begin{tabular}{l|ccc|ccc|ccc}
%        \toprule
%          &  \multicolumn{3}{c|}{1-shot test}  &  \multicolumn{3}{c|}{3-shot test} &  %\multicolumn{3}{c|}{All-shot test}  \\
%          Method & OfficeHome& PACS & VisDA& OfficeHome& PACS & VisDA& OfficeHome& PACS & %VisDA\\
%        \midrule
%        PCS 1-Shot Max &{29.32\%}	&{38.25\%}&{44.52\%}&{34.35}\%&{45.77\%}&{45.17\%} & %{41.86}\%&49.58\%&{56.76\%}\\
%        PCS 3-Shots Max & {28.56\%}&	{39.34\%}&	{44.48\%}&{35.64\%}&{50.04\%}&	%{49.38\%}&{43.11\%}&	47.64\%&	{60.02\%}\\
%        \midrule
%        PCS 1-Shot Avg &25.72\%&	35.83\%&	37.90\%& 31.45\%&	43.52\%&	%40.83\%&39.25\%&	47.86\%&	51.64\%\\
%        PCS 3-Shot Avg &25.95\%&	38.58\%&	39.00\%&33.34\%&	43.45\%&	42.78\%& %40.79\%&	50.28\%&	54.27\%\\
%        \midrule
%        Ours &{32.00\%}&	{67.25\%}&	{39.40\%}&{38.70\%}&	{79.83\%}&	%{48.10\%}&{47.34\%}&	{80.37\%}&	{57.60\%}\\
%        \bottomrule
%    \end{tabular}
%    \label{tab:ablation_main}
%\end{table*}
